Demystifying security and compatibility issues in Android Apps

Never before has any OS been so popular as Android. Existing mobile phones are not simply devices for making phone calls and receiving SMS messages, but powerful communication and entertainment platforms for web surfing, social networking, etc. Even though the Android OS offers powerful communication and application execution capabilities, it is riddled with defects (e.g., security risks, and compatibility issues), new vulnerabilities come to light daily, and bugs cost the economy tens of billions of dollars annually. For example, malicious apps (e.g., back-doors, fraud apps, ransomware, spyware, etc.) are reported [Google, 2022] to exhibit malicious behaviours, including privacy stealing, unwanted programs installed, etc. To counteract these threats, many works have been proposed that rely on static analysis techniques to detect such issues. However, static techniques are not sufficient on their own to detect such defects precisely. This will likely yield false positive results as static analysis has to make some trade-offs when handling complicated cases (e.g., object-sensitive vs. object-insensitive). In addition, static analysis techniques will also likely suffer from soundness issues because some complicated features (e.g., reflection, obfuscation, and hardening) are difficult to be handled [Sun et al., 2021b, Samhi et al., 2022].

==> alg/alg-EM.tex <==
\begin{algorithm}[H]
	\caption{The EM algorithm.}
	\label{alg:EM}
	\small{
		\begin{algorithmic}[1]
			\State Expectation step: Given the current model parameters, compute the probability distribution over the unlabeled data	$P(\vy_{l+1},...,\vy_{L+u}|L,U,\hat{\theta_{t}})$.
			\State Maximization step: Maximize the log likelihood of the \textit{pseudo complete} data to get the new parameter $\hat{\theta_{t+1}}=\textrm{arg max}_{\theta}\sum_{i=1}^{l}\textrm{log} P(\vx^{(i)}, \vy^{(i)}|\theta) + \sum_{j=l+1}^{l+u} E_{P(\vy_j|L,U,\hat{\theta_{t}})}[\textrm{log} P(\vx^{(j)},\vy^{(j)}|\theta)]$
		\end{algorithmic}	
	}
\end{algorithm}





==> alg/alg-cotrain.tex <==
\begin{algorithm}[H]
	\caption{The Co-training algorithm.}
	\label{alg:cotrain}
	\small{
		\begin{algorithmic}[1]
	    	\Statex \hspace{-5mm} \textbf{Input:} $L=\{(\vx_i, \vy_i)\}_{i=1}^l$ and $U= \{\vx_j\}_{j=l+1}^{l+u}$,
	    	\State Initially let the training sample be $L_1=L_2=\{(\vx_i, \vy_i)\}_{i=1}^l$
			\While {$U$ is not used up}
			    \State Train a view-1 model $f_1$ from $L_1$, and  a view-2 model $f_2$ from $L_2$
			    \State Apply $f_1$ and $f_2$ to the unlabeled instances in $U$
			    
			    \State Add $f_1's$ top $k$ most confident predictions to $L_2$
			    \State Add $f_2's$ top $k$ most confident predictions to $L_1$
			    \State Remove these examples from $U$
			   
			\EndWhile
		\end{algorithmic}	
	}
\end{algorithm}





==> alg/alg-main-il-back.tex <==
\begin{algorithm*}
	\caption{Learn active learning policy for low resource neural machine translation}
	\label{alg:policytrain}
	\small{
		\begin{algorithmic}
			%\Require 
			\Statex \hspace{-5mm} \textbf{Input:} large parallel corpus $D$, pre-trained multi-lingual embeddings $E$, max episodes $T$, total active learning steps $B$, mini-batch size $K$ (in every step sample $K$ data points for the agent for learning the policy), selection flag $f$ (boolean), the coin parameters $\alpha, \beta$ %, \reza{the number of variant batches $L$}
			%\Ensure 
			\Statex \hspace{-5mm} \textbf{Output:} policy $\pi$.
			%//Obtain expert trajectory
			\State {$M \gets \emptyset$} \Comment{Replay memory}
			
			\State $D^P \gets \textrm{sampleUniform}(D, 500k)$
			
			\State Fix the vocabulary based on $E$ and $D^P$
			
			\State {Initialise $\pi$  with a random policy}
			
			%	\State {Pre-train source and target word embeddings on $D^S$ and $D^T$} 
			
			%	\State {$\vphi \gets \textrm{trainModel}(D^P)$}
			
			%	\State Re-train the word embedding based on $D^S$  and $D^T$, but freeze the embedding of words appearing in $D^P$ 
			
			\For{$\tau \in {1,\dots,T}$}
			
			
			\State $\labd, \evald, \unlabd \gets \textrm{randomPartition}(D^P)$
			
			\State $\vphi \gets \textrm{trainModel}(\labd)$
			
			\State $n \gets \textrm{number of tokens of random K source sentences from } \unlabd$
			
			
			\For{$t \in {1, \dots, B}$}
			
			\State $\textrm{globalContext} \gets \overrightarrow{0}$
			
			\State $c \gets \textrm{coinToss}(\alpha)$
			\If{$c = \textrm{Head}$} \Comment{Policy evaluation} %do random partition
			
			\State $\vb \gets \textrm{select}(\unlabd, \pi, 0, K, n, \textrm{globalContext},\vphi,f)$ 
			
			\State $\vphi \gets \textrm{updateModel}(\vphi, \vb, \labd)$
			
			\State $\labd \gets \labd + \vb$
			
			\Else \Comment{Policy improvement} 
			
			%			\State $\vb_0 \gets \textrm{select}(\unlabd, \pi, 0,K, \textrm{globalContext},\vphi)$
			%			\State $\vphi_0 \gets \textrm{updateModel}(\vphi, \vb_0, \labd)$
			
			%			\For{$\ell = 1.. L$}
			%  			   \State $\vb_{\ell} \gets \textrm{select}(\unlabd, \pi, \beta,K, \textrm{globalContext},\vphi,)$
			%			   \State $\vphi_{\ell} \gets \textrm{updateModel}(\vphi, \vb_0, \labd)$
			%			\EndFor
			
			%			\State $\ell^* = \arg\max_{\ell \in \{ 0, 1, .., L\}} \textrm{BLEU}($\vphi_{\ell}, \evald$)$
			%			\State $\vphi \gets \vphi_{\ell^*}$
			
			
			\State $\vb_1 \gets \textrm{select}(\unlabd, \pi, 0,K,n, \textrm{globalContext},\vphi, f)$ 
			
			\State $\vb_2 \gets \textrm{select}(\unlabd, \pi, \beta,K,n, \textrm{globalContext},\vphi, f)$
			
			\State $\vphi_1 \gets \textrm{updateModel}(\vphi, \vb_1, \labd)$
			
			\State $\vphi_2 \gets \textrm{updateModel}(\vphi, \vb_2, \labd)$
			
			\If{BLEU($\vphi_1, \evald$)$>$BLEU($\vphi_2, \evald$)}
			
			\State $\vphi \gets \vphi_1$
			
			\State $M \gets M + (\vb_1, \vb_2, \textrm{globalContext})$
			
			\State $\textrm{globalContext} \gets \textrm{globalContext} + \textrm{Rep}(\vb_1,\vphi)$
			
			\State $\labd \gets \labd + \vb_1$
			
			\Else
			
			\State $\vphi \gets \vphi_2$
			
			\State $M \gets M + (\vb_2, \vb_1, \textrm{globalContext})$
			
			\State $\textrm{globalContext} \gets \textrm{globalContext} + \textrm{Rep}(\vb_2,\vphi)$
			
			\State $\labd \gets \labd + \vb_2$
			
			\EndIf
			\EndIf
			\EndFor
			
			\State $\pi \gets \textrm{updatePolicy}(\pi,M,\vphi)$
			
			
			\EndFor
			\State \Return { ${\pi}$}
		\end{algorithmic}
	}	
\end{algorithm*}





==> alg/alg-main-il.tex <==
\begin{algorithm}[H]
	\caption{Learning AL-NMT Policy}
	\label{alg:policytrain}
	\small{
		\begin{algorithmic}[1]
			%\Require 
			\Statex \hspace{-5mm} \textbf{Input:}  Parallel corpus $D$, $I_{\textrm{width}}$  the width
			 of the constructed search lattices, the coin parameter $\alpha$, the number of sampled  AL batches $K$
			%\Ensure 
			\Statex \hspace{-5mm} \textbf{Output:} policy $\pi$
			%//Obtain expert trajectory
			\State {$M \gets \emptyset$} \Comment{Replay Memory}
									
			\State {Initialise $\pi$  with a random policy}
			
			%	\State {Pre-train source and target word embeddings on $D^S$ and $D^T$} 
			
			%	\State {$\vphi \gets \textrm{trainModel}(D^P)$}
			
			%	\State Re-train the word embedding based on $D^S$  and $D^T$, but freeze the embedding of words appearing in $D^P$ 
			
			\For{$\mathcal{T}$ training iterations}
						
			\State $\labd, \evald, \unlabd \gets \textrm{randomPartition}(D)$
			
			\State $\vphi \gets \textrm{trainModel}(\labd)$
			
			\State $\vc_{\textrm{global}} \gets \pmb{0}$
			
			\For{$t \gets 1 \textrm{ to } T_{\textrm{HI}}$} \Comment{$\textrm{MDP}_{\textrm{HI}}$}


			\State $\mathcal{S} \gets \textrm{searchLattice}(\unlabd,I_{\textrm{width}}) $
			
			
		%	\State $c \gets \textrm{coinToss}(\alpha)$
			\If{$\textrm{coinToss}(\alpha) = \textrm{Head}$}   %do random partition
			
			\State $\vB \gets \{\textrm{samplePath}(\mathcal{S}, \vphi, \vc_{\textrm{global}},\pi, \beta)\}_{1}^K$  % \Comment{$\textrm{MDP}_{\textrm{LO}}$}
			\State $\vB \gets \vB + \textrm{samplePath}(\mathcal{S}, \vphi, \vc_{\textrm{global}},\pi, 0)$ 
			
			\State $\displaystyle{\vb \gets \arg\max_{\vb' \in \vB}\textrm{BLEU}(m_{\vphi}^{\vb'}, \evald)}$   \Comment{expert}
			
			\State $M \gets M \cup \{(\vc_{\textrm{global}},\vphi,\vB,\vb)\}$
			
			\Else
			
			\State $\vb \gets \textrm{samplePath}(\mathcal{S}, \vphi,  \vc_{\textrm{global}},\pi, 0)$ \Comment{policy}

			\EndIf
						
			\State $\labd \gets \labd + \vb$
			
			\State $\unlabd \gets \unlabd - \{\vx \textrm{ s.t. } (\vx,\vy) \in \vb\}$ % \vx_{\vb}$%\vb_{\textrm{source}}$ %\Comment{remove the source part of $\vb$ from the pool}

			\State $\vphi \gets \textrm{retrainModel}(\vphi, \labd)$
			
			\State $\vc_{\textrm{global}} \gets \vc_{\textrm{global}}  \oplus \textrm{rep}(\vb)$

			\EndFor
			
			\State $\pi \gets \textrm{updatePolicy}(\pi,M,\vphi)$
			
			
			\EndFor
			\State \Return { ${\pi}$}
		\end{algorithmic}
	}	
\end{algorithm}





==> alg/alg-policy-transfer.tex <==
\begin{algorithm}[H]
	\caption{Policy Transfer}
	\label{alg:transferpolicy}
	\small{
		\begin{algorithmic}[1]
			\Statex \hspace{-5mm} \textbf{Input:} Bitext  $\labd$, monotext $\unlabd$, pre-trained policy $\pi$
			%\Ensure 
			\Statex \hspace{-5mm} \textbf{Output:} NMT model $\vphi$
			
			
			\State \textrm{Initialise $\vphi$ with $\labd$}
			
			\State $\gc \gets \pmb{0}$
			
			\For {$t \gets 1 \textrm{ to } T_{HI}$ }
			\State $\mathcal{S} \gets \textrm{searchLattice}(\unlabd, I_{\textrm{width}})$
			
			\State $\vb \gets \textrm{samplePath}(\mathcal{S}, \vphi, \gc, \pi, 0)$
			
			\State $\labd \gets \labd + \vb$
			\State $\unlabd \gets \unlabd - \{\vx \textrm{ s.t. } (\vx,\vy) \in \vb \}$
			\State $\vphi \gets \textrm{retrainModel}(\vphi,  \labd)$
			
			%\State $\labd \gets \labd + \vb$
			
			\State $\gc \gets \gc \oplus \textrm{rep}(\vb)$
			\EndFor
			
			\State \Return $\vphi$
		\end{algorithmic}	
	}
\end{algorithm}


==> alg/alg-select.tex <==
\begin{algorithm}[H]
	\caption{samplePath (selecting an AL batch)}
	\label{alg:select}
	\small{
		\begin{algorithmic}[1]
			\Statex \hspace{-4mm} \textbf{Input:} Search lattice $\mathcal{S}$, global context $\gc$,  policy $\pi$,  perturbation probability $\beta$ %,perturbation policy $\pi_0$
			%\Ensure 
			\Statex \hspace{-4mm} \textbf{Output:} Selected AL batch $\vb$
			
			\State $\vb \gets \emptyset$
			\State  $\lc \gets \pmb{0}$	
			\For {$t \gets 1 \textrm{ to } T_{\textrm{LO}}$}	\Comment{$\textrm{MDP}_{\textrm{LO}}$}			
			%%%%%%
			\If{coinToss($\beta$) = Head}
			\State $\vx_t \gets \pi_0(\mathcal{S}[t])$ \Comment{perturbation policy}
			\Else
			\State $\vx_t \gets \arg\max_{\vx \in \mathcal{S}[t]} \pi(\gc,\lc,\vx)$
		         \EndIf
			%%%%%%
			\State $\vy_t \gets \textrm{oracle}(\vx_t)$ \Comment{getting the gold translation}
			\State $\lc \gets \lc \oplus  \textrm{rep}(\vx_t,\vy_t)$
			\State $\vb \gets \vb + (\vx_t,\vy_t)$
			%%%%%%	        
			%%%%%%		         			
			\EndFor		
			\State \Return $\vb$			
		\end{algorithmic}	
	}
\end{algorithm}





==> alg/alg-select_back.tex <==
\begin{algorithm*}
	\caption{Algorithm for data selection: select()}
	\label{alg:select}
	\small{
		\begin{algorithmic}
			\Statex \hspace{-4mm} \textbf{Input:} $\unlabd, \pi, \beta, K,n, \textrm{globalContext}, \vphi$, $f$
			%\Ensure 
			\Statex \hspace{-4mm} \textbf{Output:} $\vb$
			\State $\vb \gets \emptyset$
			\State localContext $\gets \overrightarrow{0}$
			\State $k,\textrm{totalTokens} \gets 0$
			
			\While {True}				
			\If{coinToss($\beta$) = Head}
			%%%%%%
			\State $\vx^{\textrm{best}} \gets \textrm{sampleUniform}(\unlabd,1)$
			\State $ \vy_{\vx^{\textrm{best}}} \gets \textrm{oracle}(\vx^{\textrm{best}})$
			%%%%%%
			\Else
			%%%%%%		
			\State $D'^{S} \gets \textrm{sampleUniform}(\unlabd, I)$ \Comment{$I$ is a user-defined parameter}
			\For{$\vx \in D'^S$}
			\State $ \vy_{\vx} \gets \textrm{oracle}(\vx)$
			\State $\textrm{score}(\vx) \gets \pi(\textrm{globalContext},\textrm{localContext},\textrm{Rep}(\vx,\vy_{\vx},\vphi))$
			\EndFor
			\State $\vx^{\textrm{best}} \gets \arg\max_{\vx \in D'^S} \textrm{score}(\vx)$
			%%%%%%%
			\EndIf
			\State $\vb \gets \vb + \{(\vx^{\textrm{best}},\vy_{\vx^{\textrm{best}}})\}$
			\State $\textrm{localContext} \gets \textrm{localContext} + \textrm{Rep}(\vx^{\textrm{best}},\vy_{\vx^{\textrm{best}}},\vphi)$ 
			\If{f=True}
			  \State $k=k+1$
			  \If{$k>=K$}
			    \State break
			  \EndIf
			  
			\Else
			  \State totalTokens = totalTokens + length ($\vx^{\textrm{best}}$)
			  \If{$\textrm{totalTokens} >= n$}
			    \State break
			  \EndIf
			
			\EndIf
			\EndWhile		
			\State \Return $\vb$
			
		\end{algorithmic}	
	}
\end{algorithm*}





==> alg/alg-selftrain.tex <==
\begin{algorithm}[H]
	\caption{The Self training algorithm.}
	\label{alg:selftrain}
	\small{
		\begin{algorithmic}[1]
	    	\Statex \hspace{-5mm} \textbf{Input:} $L=\{(\vx_i, \vy_i)\}_{i=1}^l$ and $U= \{x_j\}_{j=l+1}^{l+u}$.
			\While {$U$ is not empty}
			    \State Train $f$ from $L$ using supervised learning objective
			    \State Apply $f$ to the unlabeled instances in $U$
			    \State Remove a subset $S$ from $U$
			    \State Add $\{(\vx, f (\vx))|\vx \in S\}$ to $L$
			   
			\EndWhile
		\end{algorithmic}	
	}
\end{algorithm}





==> alg/alg-update-model.tex <==
\begin{algorithm}[H]
	\caption{Algorithm for updating model: updateModel()}
	\label{alg:updatemodel}
	\small{
		\begin{algorithmic}
			\Statex \hspace{-4mm} \textbf{Input:} $\phi, \vb, D^P$
			%\Ensure 
			\Statex \hspace{-4mm} \textbf{Output:} $\phi'$
			\State \textrm{Initialise $\phi'$ with $\phi$}
			\State Sample $D^{tmp}$ from $D^P$ randomly
			\State $\phi' \gets trainModel(D^{tmp}+\vb)$
			% \State $D^P \gets D^P + \vb$
			\State \Return $\phi'$
		\end{algorithmic}	
	}
\end{algorithm}




==> alg/alg-update-policy.tex <==
\begin{algorithm}[H]
	\caption{Algorithm for updating policy: updatePolicy()}
	\label{alg:updatepolicy}
	\small{
		\begin{algorithmic}
			\Statex \hspace{-5mm} \textbf{Input:} replay memory $M$, old policy $\pi$, ${\vphi}$
			%\Ensure 
			\Statex \hspace{-5mm} \textbf{Output:} new policy $\pi$.
			
			\State $\textrm{goodbatch, badbatch, globalContext} \gets \textrm{latestTuple}(M)$
			
			\State $\textrm{goodscore, badscore} \gets 0$
			
			\State localContext $\gets \overrightarrow{0}$
			
			\For{$(s,t) \in \textrm{goodbatch}$}
			
			\State $\textrm{goodscore} \gets \textrm{goodscore} + \pi (\textrm{globalContext, localContext, Rep}(s,t,{\vphi}))$
			
			\State $\textrm{localContext} \gets \textrm{localContext} + \textrm{Rep}(s,t,{\vphi})$
			
			\EndFor
			
			\State localContext $\gets \overrightarrow{0}$
			
			\For{$(s,t) \in \textrm{baddbatch}$}
			
			\State $\textrm{badscore} \gets \textrm{badscore} + \pi (\textrm{globalContext, localContext, Rep}(s,t,{\vphi}))$
			
			\State $\textrm{localContext} \gets \textrm{localContext} + \textrm{Rep}(s,t,{\vphi})$
			
			\EndFor
			
			\While{not converged}
			\State $\pi_\theta \gets \pi_\theta + \nabla_{\pi_\theta} (\textrm{goodscore} - \textrm{badscore})$
			\EndWhile
			
			\State \Return ${\pi}$
		\end{algorithmic}	
	}
\end{algorithm}


==> v_include.tex <==
\chapter*{Thesis including published works declaration}
I hereby declare that this thesis contains no material which has been accepted for the award of any other degree or diploma at any university or equivalent institution and that, to the best of my knowledge and belief, this thesis contains no material previously published or written by another person, except where due reference is made in the text of the thesis. 

This thesis includes 3 original papers published/submitted in peer reviewed journals. The core theme of the thesis is intelligent question and answering in software Q\&A community. 
The ideas, development and writing up of all the papers in the thesis were the principal responsibility of myself, the student, working within the Monash University under the supervision of Prof. John Grundy and Dr. Xin Xia.

% In the case of Chapter 3,4,5 my contribution to the work involved the following:
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         \textbf{Thesis Chapter} & \textbf{Publication Title} & \textbf{Status} & \textbf{Nature and \% of student contribution} & \textbf{Co-author name(s) Nature and \% of Co-author’s contribution} & \textbf{Co-author(s), Monash student Y/N} \\
%          % 3 & Learning cascaded latent variable models for biomedical text classification & Published & 85\%. Concept, experiments and writing the paper. & 1) Wray, algorithm check 10\% 2)Reza, draft check 5\% & No \\
%          % \hline 
%          % 3 & Deep learning for recognition of invasive fungal disease from chest computed tomography in haematology-oncology patients & Published & & & \\
%          % 4 & & & & & \\
%          % 5 & & & & & \\
%          % 6 & & & & & \\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}
% I have / have not renumbered sections of submitted or published papers in order to generate a consistent presentation within the thesis.

I hereby certify that the above declaration correctly reflects the nature and extent of the student’s and co-authors’ contributions to this work. In instances where I am not the responsible author I have consulted with the responsible author to agree on the respective contributions of the authors. 

% \vspace{20mm}
\textbf{Student signature:}  \hspace{50mm} \textbf{Date: 2021/10/19}

\vspace{17mm}
\textbf{Main Supervisor signature:} \hspace{50mm} \textbf{Date: 2021/10/19}
